Exploiting The Laws of Order in Smart Contracts

We investigate a family of bugs in blockchain-based smart contracts, which we call event-ordering (or EO) bugs. These bugs are intimately related to the dynamic ordering of contract events, i.e., calls of its functions on the blockchain, and enable potential exploits of millions of USD worth of Ether. Known examples of such bugs and prior techniques to detect them have been restricted to a small number of event orderings, typicall 1 or 2. Our work provides a new formulation of this general class of EO bugs as finding concurrency properties arising in long permutations of such events. The technical challenge in detecting our formulation of EO bugs is the inherent combinatorial blowup in path and state space analysis, even for simple contracts. We propose the first use of partial-order reduction techniques, using happen-before relations extracted automatically for contracts, along with several other optimizations built on a dynamic symbolic execution technique. We build an automatic tool called ETHRACER that requires no hints from users and runs directly on Ethereum bytecode. It flags 7-11% of over ten thousand contracts analyzed in roughly 18.5 minutes per contract, providing compact event traces that human analysts can run as witnesses. These witnesses are so compact that confirmations require only a few minutes of human effort. Half of the flagged contracts have subtle EO bugs, including in ERC-20 contracts that carry hundreds of millions of dollars worth of Ether. Thus, ETHRACER is effective at detecting a subtle yet dangerous class of bugs which existing tools miss.

==> approach-overview.tex <==
\subsection{Approach Overview}

The technical barrier to finding reordering bugs
is the large number of potential reorderings.
A typical contract has perhaps 20 distinct functions, each of which
can be called by different accounts with varying arguments.  Accordingly, a
single (relatively short) sequence of calls to the contract's
functions may have billions of reorderings.  Inspecting even a single
sequence of function calls is thus infeasible.
%\footnote{For instance, sequence of 6 functions calls, each with at most 2 inputs results in $C_{(20\cdot 2\cdot 6)!}^{6!} \approx 2^{38} $}

We develop a practical tool, \toolname, that checks if a contract has reordering bugs.
In comparison to a na\"ive strategy, we employ three major
optimizations: a reduction in the number of analyzed functions, a reduction in
the number of possible function sequences, and the construction of important
function inputs.
%
The algorithm works as follows.
First, we filter out all functions that do not impact the blockchain state as
they cannot trigger reordering bugs. For the remaining functions we
build a \emph{happens-before} relation that establishes a partial
order on possible function calls. Finally, we construct all possible sequences of
function calls (of parametric bounded length) and check if any of their reorderings results
in a different state. Due to the happens-before relation, the search space of
possible sequences and their reorderings is significantly reduced.
\marginpar{Aquinas asks: do we want to discuss the construction of important function inputs here?}

We use symbolic execution
to find the significant functions, their inputs, and  their happens-before
relations; and an independent Ethereum Virtual Machine (EVM) executing unit to
efficiently test if different function calls result in identical global states,
along with a number of heuristics that help speed the search.
\toolname allows the user to specify certain bounds for the search parameters,
but in practice takes around 20 minutes to process a contract.




\begin{comment}

function permutations is intractably large.
Even a naive strategy is to enumerate all permutations and test --- for even
simple contracts with say $20$ functions, this exploration takes weeks!
\textbf{Dealing with intentional randomness?}
We explain how our tool reduces this effort to a few hours and finds
a number of subtle behaviors which we deem to be buggy.


\end{comment}


==> approach.tex <==
\subsection{Design}
\label{sec:design}

A function of a contract invoked with one set of inputs, may result in
a different final state of the blockchain than the same function
invoked with a different set. We can observe a similar behaviour with
the address from which the function is invoked and the value sent in
the transaction.  In practice, we have observed that an invocation
identified by the function invoked, inputs, address of the sender and
the value sent will mostly result in the same final state of the
blockchain given the same initial state. Therefore, we define an
invocation as $\langle \texttt{fn}, \texttt{ctx} \rangle$ where fn is
the function of the contract and ctx is the context of the invocation
which includes all the three other parameters. Thus, a trace of such
invocations constitute an execution.

Our approach is to assume that the security analyst has access to a
{\em benign testsuite} that grounds a subset of the legitimate
behavior of the contract. We expect that contract writers can provide
this information directly for the analysis. In such case, a naive way
to find the reordering bugs would be to check the output state of the
blockchain for all the permutations of a particular benign trace. When
a permuted execution leads to a different state of the blockchain than
the benign execution, we flag the execution as a reordering bug.

However, the reader may notice that the complexity of the naive method
is exponential.  In reality, one does not need to check for all
possible permutations of a benign trace. Some invocations might never
happen after another, For instance, the
$\langle \texttt{submitProposal}, \texttt{u1} \rangle$ always happens
before $\langle \texttt{voteProposal}, \texttt{(u1)} \rangle$ in the
example contract i.e., if the invocations are executed in reverse
order they always throw regardless of the state of the
blockchain. This relation between the two invocations relieves the
number of permutations of an execution containing these invocations
which are to be checked, already by a factor of two.

Therefore, to aid our analysis, we define a relation called
\em{Happens} \em{Before} and also a way to retieve this relation for a
particular set of invocations. Then, we use this relation to reduce
our final search space in finding the reordering bugs.  However,
sometimes the traces in testsuite are not adequate to find the bugs,
For instance, by permuting the set of benign executions we will miss
the executions which are not in the testsuite but are still possible
i.e., the executions which are unexpected.
we generate our own traces and check if any two permuted traces result in different outputs.\\

\paragraph{\textbf{Challenges:}}
\begin{itemize}
		\item How do we build our HB relation effectively given the nodes?
		\item How do we find the reordering bugs once we have
                  the HB relation?
	\end{itemize}	



==> background.tex <==
Ethereum is a public distributed computing platform based on blockchain technology. It features a crypto currency called Ether, similar to bitcoin, and smart-contract functionality. Two types of accounts can be created on an Ethereum interface, a normal or an external user controlled account and a smart contract account. A smart contract is a piece of code written in Ethereum supported languages like Solidity and Serpent. Smart contracts are deployed on the blockchain by creating a contract account which is represented by it's address, contract code, contract storage and account balance unlike a normal account with only address and balance. Both the accounts can create transactions and submit them to the Ethereum network, which are mined or executed by the miners on the network. Miners execute the submitted transactions and solve a mathematical puzzle in order to commit their executions to the blockchain in the form of a block. A block therefore, constitutes of all the transactions executed by the miner in their execution order along with logs, block number and various other fields which give information related to the transactions inside the block and also about it's previous block. The transactions on Ethereum encapsulate semantics which help in using the smart contract functionalities in addition to sending money from one account to another. A smart contract consists of functions, both public and private, a constructor which is called only once when deploying the contract.Once deployed on an account on blockchain, it is stored as bytecode and is assigned a storage which stores all the global variables of the contract. All the local variables of a contract function are stored in memory when the transaction invoking the function is being executed by a miner. \textbf{Once deployed on blockchain a contract code cannot be changed}. 

Every transaction execution requires some amount of gas. The minimum amount of gas is 21000, used while merely sending ether to another account. The amount of gas required for a transaction can be estimated beforehand, and must be specified while sending a transaction. The amount of ether which needs to be spent for execution of a transaction is calculated from gas x gasPrice, here gasPrice is the amount one is willing to pay for one unit of gas to execute their transaction and is used to rank the transactions by the miners while executing. Incase if the gas is exhausted or the sender's account doesn't have enough money to execute a transaction, the transaction is rolled back and the amount of ether used up until that point would be deducted from sender's account. A transaction consists of following fields.
\begin{enumerate}
	\item \textbf{nonce:} Serial number of the transaction from an account.
	\item \textbf{gasLimit:} The maximum amount of expected gas for executing the transaction.
	\item \textbf{gasPrice:} The amount sender is willing to pay per unit of gas.
	\item \textbf{Toaddress:} The address to which transaction is being sent.
	\item \textbf{value:} The amount of ether to be sent apart from transaction charges.
	\item \textbf{init:} This carries the byte code of a smart contract when it is about to be deployed and is only present in such transactions.
	\item \textbf{data:} This has the information related to invocation of a contract method like function hash, inputs to the function etc.,
	\item \textbf{signature:} This consists of signature of the transaction to verify the sender.          
\end{enumerate} 

Both the externally owned and smart contract accounts can invoke contract's methods by creating and submitting a transaction with the data field consisting of the function information.


==> bounty.tex <==
\begin{figure*}[t]
\centering
\begin{tabular}{cc}
\begin{minipage}{0.50\linewidth}
\begin{lstlisting}[mathescape=true,language=Solidity]
contract Bounty {
    bool public bounty_paid = false;
    uint256 public count_donors = 0;
    mapping (address => uint256) public balances;
    mapping (address => bool) public has_donated;
    mapping (address => bool) public has_voted;
    address public proposed_beneficiary = 0x0;
    uint256 public votes_for = 0;
    uint256 public votes_against = 0;
    bytes32 hash_pwd = ...

    modifier onlyDonor {
        require(!bounty_paid);
        require(has_donated[msg.sender]);
        _;
    }

    function payout(string _password) {
        require(keccak256(_password) == hash_pwd);
        require(!bounty_paid);
        require(proposed_beneficiary != 0x0);
        require(votes_for > votes_against);
        require(votes_for+votes_against > count_donors*8/10);
        bounty_paid = true;
        proposed_beneficiary.transfer(this.balance);
    }

    function propose_beneficiary(address _proposed) onlyDonor {
        proposed_beneficiary = _proposed;
        votes_for = 0;
        votes_against = 0;
    }
\end{lstlisting}
\end{minipage}
&
\begin{minipage}{0.45\linewidth}
\begin{lstlisting}[mathescape=true,language=Solidity]
    function vote_beneficiary(string _vote) onlyDonor {
        require(!has_voted[msg.sender]);
        require(proposed_beneficiary != 0x0);
        if (keccak256(_vote) == keccak256("yes")) {
            votes_for += 1;
            has_voted[msg.sender] = true;
        }
        if (keccak256(_vote) == keccak256("no")) {
            votes_against += 1;
            has_voted[msg.sender] = true;
        }
    }

    function refund() onlyDonor {
        has_donated[msg.sender] = false;
        count_donors -= 1;
        uint256 eth_to_withdraw = balances[msg.sender];
        balances[msg.sender] = 0;
        msg.sender.transfer(eth_to_withdraw);
    }

    function () payable {
        require(!bounty_paid);
        require(count_donors < 51);
        require(msg.value >= 0.1 ether);
        if (!has_donated[msg.sender]) {
            has_donated[msg.sender] = true;
            count_donors += 1;
        } 
        balances[msg.sender] += msg.value;
    }
}
\end{lstlisting}
\end{minipage}
\end{tabular}
\caption{\texttt{Bounty} contract.}
\label{fig:bounty} 
\end{figure*}


==> creditDao.tex <==
\begin{figure*}[t]
\centering
\begin{tabular}{cc}
\begin{minipage}{0.50\linewidth}
\begin{lstlisting}[mathescape=true,language=Solidity]
/*
.
.
*/


contract CreditDAO {
    /*
    Constructor and intialized global variables
    */

    // Election part
    function createNewElections() {
        require(elections[nextElectionIndex - 1].endBlock + mandateInBlocks < block.number);

        elections[nextElectionIndex].startBlock = block.number;
        elections[nextElectionIndex].endBlock = block.number + blocksPerMonth;
        /*
        ..
        */
        nextElectionIndex++;
    }    
        

    function sumbitForElection() {
        require(elections[nextElectionIndex - 1].endBlock > block.number);
        require(!elections[nextElectionIndex - 1].candidates[msg.sender]);
        /*
        Add the candidate to different datastructures
        */
        elections[nextElectionIndex - 1].candidates[msg.sender] = true;
        
    }
\end{lstlisting}
\end{minipage}
&
\begin{minipage}{0.45\linewidth}
\begin{lstlisting}[mathescape=true,language=Solidity]
    function vote(address _participant) {
        require(elections[nextElectionIndex - 1].endBlock > block.number);
        
       /*
       ..
       */
        require(!elections[nextElectionIndex - 1].userHasVoted[msg.sender]);
        elections[nextElectionIndex - 1].userHasVoted[msg.sender] = true;
        /*
        ..
        */
    }

    function finishElections(uint _iterations) {
        require(elections[nextElectionIndex - 1].endBlock < block.number);
        require(!elections[nextElectionIndex - 1].electionsFinished);

        uint curentVotes;
        
        /*
         Find the person with maximum votes and reward them
        */
        elections[nextElectionIndex - 1].electionsFinished = true;

        /*
        ..
        */
    }

/*
..
*/
\end{lstlisting}
\end{minipage}
\end{tabular}
\caption{\texttt{CreditDao}}
\label{fig:CreditDao} 
\end{figure*}


==> eval-linear.tex <==
\subsection{\oraclize}
\label{sec:line-relat-bugs}

\paragraph{Experimental Setup} 
To process a single contract, \oraclize requires a full list of transactions to and from the contract. However, obtaining such a list from the common Ethereum client \texttt{geth} is exceptionally slow. Instead, in the setup phase we create a database of all transactions that occurred on the blockchain until the block number 5,400,000. The database  holds 197,939,546 transactions in total, and allows easy access to all the transactions sent and received by a specific contract.
%
%
By inspecting the transactions send by Oraclize, we identify 1,152 unique contracts to which the service has replied. We filter out contract that have low number of calls to Oraclize or  low percentage of Oraclize queries. As a result, there are 423 contracts left (154 with Solidity code) -- these contracts are further processed in parallel by \oraclize.
%

\begin{comment} 
By inspecting the transactions sent to two Oraclize address resolver contracts\footnote{With addresses \texttt{0x1d3b2638a7cc9f2cb3d298a3da7a90b67e5506ed} and \texttt{0x1d11e5eae3112dbd44f99266872ff1d07c77dce8}.}, we identify five Oraclize contracts\footnote{With addresses \texttt{0x001a589dda0d6be37632925eaf1256986b2c6ad0, 0x3375ee30428b2a71c428afa5e89e427905f95f7e, 0x3dbdc81a6edc94c720b0b88fb65dbd7e395fdcf6, 
0x6f28b146804dba2d6f944c03528a8fdbc673df2c, 0x88e1315687aec48a72786c6b3b3f075208b62713}.}. 
Further analysis of the events raised by the five contracts, reveals 1152 unique contracts that are processed in parallel by \oraclize. 
\end{comment}

\vspace{5pt}
\paragraph{Performance}
On average the tool requires 54 mins to process a single contract on
one CPU core. The processing time among non-flagged contracts is
fairly constant because the fuzzer is set to generate and check
identical number of random traces.
%
The inspected contracts made on average 947 queries to Oraclize, the minimal number of queries is 1, the maximal is 132,713, while the median is 3. 

\vspace{5pt}
\paragraph{Results}
%
Due to the random nature of the fuzzer, not all buggy contracts are
flagged in a single run of the tool\footnote{The chance of detecting a
  buggy contract increases by incrementing the number of random traces
  in the fuzzer.}.  After running the tool a few times on all 423
contracts, 47 distinct contracts (approximately 11\%) are flagged by
the tool.  Among them, 28 have Solidity source code. We manually
inspect these contracts and try identify the pieces of code that
result in bugs.
%We confirm the correctness of the tool as all YY flagged contracts contain a bug, thus the tool  produced only true positives. 
Among the 28 contracts, we found 23 true positives and 5 false positives (see  Appendix~\ref{sect:appendix:oraclize}).



\vspace{5pt}

\end{itemize}



==> eval-stats.tex <==
\subsection{Statistics on the Flagged Contracts}
\label{sec:stats}

% \is{I suggest to get some plots (distributions, histograms etc)
%   clssifygin our contracts, Oraclize-related and HB-related with a the
% following aspects, to show that ``important'' instances are affected.
% All this information can be taken from Etherscan.}

\begin{itemize}

\item $785$ contracts out of $789$ flagged by \toolname, are still live on Ethereum
blockchain  and only $4$ have been killed until blocknumber $5,400,000$.
$620$($78.5\%$) contracts out of $789$ have been created after the blocknumber
$4,000,000$. The number contracts flagged by \toolname is increasing steadily
with blocknumber.

\item These contracts flagged currently hold around $307$ ether i.e.,$240,688$
USD  calculated at $784$ USD/eth. However, these contracts together held a
maximum of  $703,676$ ether  in their lifetime i.e., approx $551$ million USD
calculated at the same price.

\item $1,649,192$ transactions have been processed by these contracts until
blocknumber  $5,400,000$. The highest number of transactions by a single
contract is $771,918$ and  is flagged for the ERC bug explained in
section~\ref{sec:motivation}. $623$ contracts ($78.96\%$)  have atleast one
transaction i.e., have been used in their lifetime. 

% \item Age and lifetime: when was the contract last active, and for how
%   long did is serve, \ie, end date - start date).

% \item How much money did the contracts accumulate by now (there are
%   several with 20-30K USD on them).

% \item How much money did the contract process (net sum of all
%   transactions' amounts) during its lifetime.

% \item The overall number of transactions --- some contract could have
%   a very interesting life with 6000-7000 transactions altogether, we
%   should tell how many of such did we discover to be buggy.

\end{itemize}


==> fig-esem.tex <==
\begin{figure}[t]
\centering
{\footnotesize{
\begin{mathpar}
\inferrule*[Lab=Call]
{
M[\pc] = \opn{CALL}
\and
\bstate[\Id][\Bal] \geq z
\\
s = \Id' \cdot \fn \cdot z \cdot \args \cdot s'
\and
a = \angled{M, \Id, \pc + 1, s', m}
\\
M' = \bstate[\Id'][\fn]
\\
m' = \set{\Sender \mapsto \Id; \To \mapsto \Id'; \Value \mapsto z; \fname \mapsto \fn; \Data \mapsto \args}
\\
\bstate' = \bstate[\Id][\Bal \mapsto \bstate[\Id][\Bal] - z]
\quad
\bstate'' = \bstate'[\Id'][\Bal \mapsto \bstate'[\Id'][\Bal] + z]
}
{
\angled{\angled{M, \Id, \pc, s, m} \cdot A, \bstate}
%
  \stepc
%
\angled{\angled{M', \Id', 0, \epsilon, m'} \cdot a \cdot A, \bstate''}
} 
%     
\and
%
\inferrule*[Lab=ReturnNonEmp]
{
M[\pc] = \opn{RETURN}
\\
a' = \angled{M', \Id', \pc', s', m'}
}
{
\angled{\angled{M, \Id, \pc, v \cdot s, m} \cdot a' \cdot A, \bstate}
%
  \stepc
%
\angled{\angled{M', \Id', \pc', v \cdot s', m'}  \cdot A, \bstate}
} 
%
\and
%
\inferrule*[Left=ReturnEmp]
{
M[\pc] = \opn{RETURN}
}
{
\angled{\angled{M, \bullet, \pc, \bullet, \bullet} \cdot \epsilon, \bstate}
%
  \stepc
%
\angled{\epsilon, \bstate}
} 
%
\and
%
\inferrule*[Lab=SStore]
{
M[\pc] = \opn{SSTORE}
\and
\bstate' = \bstate[\Id][\fld \mapsto v]
}
{
\angled{\angled{M, \Id, \pc, \fld \cdot v \cdot s, m} \cdot A, \bstate}
%
  \stepc
%
  \angled{\angled{M, \Id, \pc+1, s, m} \cdot A, \bstate'} }
%
\vspace{-10pt}
%
\end{mathpar}
}}
\caption{Selectet rules of \elite operational semantics. }
\label{fig:esem}
\end{figure}


==> language.tex <==

\section{A Toy Language for Smart Contracts}
\label{sec:toy-language-smart}

We now describe Featherweight Solidity---a toy formal language for
smart contracts, which we are going to employ for identifying
concurrency-related issues.


==> lstcoq.tex <==
% colors
\definecolor{shadecolor}{gray}{1.00}
\definecolor{darkgray}{gray}{0.30}
\definecolor{violet}{rgb}{0.56, 0.0, 1.0}
\definecolor{forestgreen}{rgb}{0.13, 0.55, 0.13}

% Col language definition
\lstdefinelanguage{Coq} {
mathescape=true,						
texcl=false,
morekeywords=[1]{
  Add,
  All,
  Arguments,
  Axiom,
  Bind,
  Canonical,
  Check,
  Close,
  CoFixpoint,
  CoInductive,
  Coercion,
  Contextual,
  Corollary,
  Defined,
  Definition,
  Delimit,
  End,
  Example,
  Export,
  Fact,
  Fixpoint,
  Goal,
  Graph,
  Hint,
  Hypotheses,
  Hypothesis,
  Implicit,
  Implicits,
  Import,
  Inductive,
  Lemma,
  Let,
  Local,
  Locate,
  Ltac,
  Maximal
  Module,
  Morphism,
  Next,
  Notation,
  Obligation,
  Open,
  Parameter,
  Parameters,
  Prenex,
  Print,
  Printing,
  Program,
  Projections,
  Proof,
  Proposition,
  Qed,
  Record,
  Relation,
  Remark,
  Require,
  Reserved,
  Resolve,
  Rewrite,
  Save,
  Scope,
  Search,
  Section,
  Show,
  Strict,
  Structure,
  Tactic,
  Theorem,
  Unset,
  Variable,
  Variables,
  View,
  inside,
  outside
},
morekeywords=[2]{
  as,
  cofix,
  else,
  end,
  exists,
  exists2,
  fix,
  for,
  forall,
  fun,
  if,
  in,
  is,
  let,
  match,
  nosimpl,
  of,
  return,
  struct,
  then,
  vfun,
  with
},
morekeywords=[3]{Type, Prop, Set, True, False},
morekeywords=[4]{
  after,
  apply,
  assert,
  auto,
  bool_congr,
  case,
  change,
  clear,
  compute,
  congr,
  cut,
  cutrewrite,
  destruct,
  elim,
  field,
  fold,
  generalize,
  have,
  heval, 
  hnf,
  induction,
  injection,
  intro,
  intros,
  intuition,
  inversion,
  left,
  loss,
  move,
  nat_congr,
  nat_norm,
  pattern,
  pose,
  refine,
  rename,
  replace,
  revert,
  rewrite,
  right,
  ring,
  set,
  simpl,
  split,
  suff,
  suffices,
  symmetry,
  transitivity,
  trivial,
  unfold,
  unlock,
  using,
  without,
  wlog,
  autorewrite
},        
morekeywords=[5]{
  assumption,
  by,
  contradiction,
  done,
  exact,
  lia,
  gappa,
  omega,
  reflexivity,
  romega,
  solve,
  tauto,
  discriminate,
  unsat
},
morecomment=[s]{(*}{*)},
morekeywords=[6]{do, first, try, idtac, repeat},
showstringspaces=false,
morestring=[b]",
% Size of tabulations
tabsize=3,							
% Enables ASCII chars 128 to 255
extendedchars=true,  		 		
% Case sensitivity
sensitive=true, 
% Automatic breaking of long lines
breaklines=false,
% Default style fors listings
%basicstyle=\scriptsize\ttfamily,
basicstyle=\footnotesize\ttfamily,
% Position of captions is bottom
captionpos=b,							
% Full flexible columns 
columns=[l]fullflexible,
% Style for (listings') identifiers
identifierstyle={\color{black}},
% Style for declaration keywords
keywordstyle=[1]{\color{violet}},
% Style for gallina keywords
keywordstyle=[2]{\color{forestgreen}},
% Style for sorts keywords
keywordstyle=[3]{\color{forestgreen}},
% Style for tactics keywords
keywordstyle=[4]{\color{blue}},
% Style for terminators keywords
keywordstyle=[5]{\color{red}},
%Style for iterators
keywordstyle=[6]{\color{violet}},
% Style for strings
stringstyle=,
% Style for comments
commentstyle=\it\ttfamily\color{Bittersweet},
% Style for lines numbering
numberstyle=\tiny,
literate={\\/}{{$\vee$}}1
         {/\\}{{$\wedge$}}1
         {:->}{{$\mapsto~$\!}}1
         {<--}{{$\asgn~$}}1
         {\\in}{{$\in~$}}1
         {++}{{$+\!+\!~$}}1
         {->}{{$\to~$}}1
         {forall}{{$\forall~$}}1
         {exists}{{$\exists~$}}1
         {=>}{{$\Rightarrow~$}}1
         {\\+}{{$\!\join\!~$}}1
}

\lstdefinestyle{Coq}{language=Coq}

==> overview.tex <==
\section{Overview and Main Ideas}
\label{sec:overview}

In this section, we outline the rationale and intuition for the
concurrency-related issues in smart contracts.

\subsection{Atomicity}
\label{sec:logical-atomicity}

Here, we present the \scode{BlockKing} contract and explain the idea
with matching calls/returns.
%
\is{I will do it later, as this part is more or less known.}

\subsection{Happens-before and determinism}
\label{sec:oper-order-determ}

A contract's implementation imposes an intrinsic \emph{happens-before}
order (\HB)~\cite{Lamport:CACM78,Mansky-al:CPP17} on the invocations
of its functions, by specific accounts, and with specific parameters
(\ie, messages). While there is no explicit synchronization mechanism
in the contract machinery, the clients can engineer it in an ad-hoc
way by relying on the transactional behavior of contracts invocations.

As a working example, let us consider the contract \scode{Bounty} in
Figure~\ref{fig:bounty}. This contract includes several modes of
interaction that potential clients can engage into. For instance, a
client that runs the default (``main'') function with a suitable
amount of Ether becomes a ``donor'', thus, gaining the permission to
invoke other methods of the contract. The permission mechanism, in
this particular example, is encoded Solidity's mechanism of
\scode{require}-assertions and \scode{modifier}-annotations that both
allow for dynamic checking of certain conditions during the contract's
execution.

From the implementation of the contract, we can see that, for
instance, the function \scode{payout} cannot be executed before
certain invocation of \code{propose_beneficiary} has been made (by
this or some other sender), as otherwise the following check in its
body will fail:

\vspace{5pt}
\begin{center}
\code{require(proposed_beneficiary != 0x0);}  
\end{center}
\vspace{5pt}

\noindent
%
The same holds for some other methods. The \emph{static}
over-approximation of the overall relation, which does not
difrerentiate between values of call parameters, but only between
specific functions \is{and, therefore, is too coarse-grained and
  having false positives} is presented in Figure~\ref{fig:bounty-hb}.


What does having such a relation between dynamic function invocations
achieve?
%
In the spirit of concurrency-inspired reasoning, the transitive
closure of the $\hb$ relation, once constructed\footnote{We will
  elaborate below on how to construct this relation.} defines the
order of contract operations ``as it was meant to be'' by the
programmer.
%
That is, operations that are not \HB-ordered can be scheduled to be
executed by the protocol in \emph{any} order. And this is where the
real races/nondeterministic behaviors can take place, due to the
overall non-deterministic scheduling of transactions to be included
into blocks.

For example, imagine that two operation invocations (\ie, invocations
of methods of a specific contract instance, with some fixed
parameters), A and B are not \HB-related, \ie, as the contract is
defined, either can go before another.
%
This is good, as long as the effect of \emph{swapping} these two
operations to the state of the contract is the same as without doing
so.
%
As an example, let us consider two independent calls of the operation
\code{vote_beneficiary} of the contract \code{Bounty} from
Figure~\ref{fig:bounty}. The code is straightforward enough to see
that for any two different donors, who have not yet cast their votes,
permuting two successful calls will not cause any harm, as the effect
of one would not affect the effect of another. This, however, might
not always be the case: swapping two operations might result in
neither of them failing, yet delivering a different effect to the
contract state. We consider such situations races, and our goal is to
detect them, given a constructed dynamic \HB-structure.

\input{bounty}

\begin{figure}[t]
  \fbox{
\begin{varwidth}{\dimexpr\textwidth+2\fboxsep-2\fboxrule\relax}
\centering
  \includegraphics[width=0.465\textwidth]{pics/hb-bounty.pdf}  
\end{varwidth}}
\caption{A static over-approximation of the \emph{hb} relation for the
  \texttt{Bounty} smart contract.}
\label{fig:bounty-hb} 
\end{figure}

In the next section, we introduce the necessary formal definitions,
and presents algorithms and data structures for computing the
necessary information about dynamic contract executions.


==> oyente_FP.tex <==
\begin{figure}[t]
\centering
\begin{lstlisting}[mathescape=true,language=Solidity,basicstyle=\scriptsize\ttfamily]

contract PresaleBREMP is Token {    
    function withdraw() public {
        require(presaleOwner == msg.sender || owner == msg.sender);
        msg.sender.transfer(this.balance);
    }
    
    function killMe() public onlyOwner {
        presaleOwner.transfer(this.balance);
        selfdestruct(owner);
    }
}
\end{lstlisting}
%\end{minipage}
%\end{tabular}
\captionof{figure}{Contract flagged by oyente. The withdraw function when called by different accounts owner and presaleOwner, results in different ether flows.}
%\caption{\texttt{Buggy} contract.}
\label{fig:oyenteFP} 
%\end{figure*}
\end{figure}
%\end{multicols}

==> problem.tex <==
\subsection{Problem \& Our Approach}
%

A blockchain can contain thousands of transactions invoking different
functions in a contract. The semantics of Ethereum---and the other
major smart contract platforms to date---does not provide programmatic
methods to manage transaction ordering: miners have complete freedom
to select which transactions, and in which order, make up a
block.  



